Characterizing Coherent Integrated Photonic Neural Networks under Imperfections

Integrated photonic neural networks (IPNNs) are emerging as promising successors to conventional electronic AI accelerators as they offer substantial improvements in computing speed and energy efficiency. In particular, coherent IPNNs use arrays of Mach-Zehnder interferometers (MZIs) for unitary transformations to perform energy-efficient matrix-vector multiplication. However, the underlying MZI devices in IPNNs are susceptible to uncertainties stemming from optical lithographic variations and thermal crosstalk and can experience imprecisions due to non-uniform MZI insertion loss and quantization errors due to low-precision encoding in the tuned phase angles. In this paper, we, for the first time, systematically characterize the impact of such uncertainties and imprecisions (together referred to as imperfections) in IPNNs using a bottom-up approach. We show that their impact on IPNN accuracy can vary widely based on the tuned parameters (e.g., phase angles) of the affected components, their physical location, and the nature and distribution of the imperfections. To improve reliability measures, we identify critical IPNN building blocks that, under imperfections, can lead to catastrophic degradation in the classification accuracy. We show that under multiple simultaneous imperfections, the IPNN inferencing accuracy can degrade by up to 46%, even when the imperfection parameters are restricted within a small range. Our results also indicate that the inferencing accuracy is sensitive to imperfections affecting the MZIs in the linear layers next to the input layer of the IPNN.

==> Long_Path_Sel.tex <==
Variations in CNFET process parameters affect the propagation delay of logic gates in a netlist, and these faults can be detected using a test set that propagates transitions though the fault sites. In the conventional approach, the minimum-slack testable path through a fault site is used for pattern generation. However, under process variations, the delay through each path changes, and thus another path through the fault site may have lesser slack than the original selected long path. As a result, SDDs might not be propagated through the minimum-slack paths and therefore remain undetected. \textcolor{black}{For example, in Fig. \ref{circuitdiag}, suppose $P_1$ ($P_2$) is the critical path  through the fault site under $RVS_1$ ($RVS_2$). If $P_1$ has a larger nominal delay, the commercial ATPG tool will sensitize $P_1$ for both these scenarios ($RVS_1$ and $RVS_2$), and thus some SDDs may be undetected in $RVS_2$.} However, in the proposed method, we consider the non-linear CNFET process variations to shortlist multiple long paths through each gate in the netlist under different random process variation scenarios. As a result, the test patterns obtained using the proposed Variation-Aware Delay Fault (VADF) testing method are more likely to propagate an SDD through the longest path, even in the presence of process variations. \textcolor{black}{Therefore, in Fig. \ref{circuitdiag}, VADF test patterns can sensitize both $P_1$ and $P_2$.} Along with the gate-level netlist, VADF takes the following inputs to achieve this:
\begin{itemize}
    \item $\rho_{max}$: The maximum number of paths to be considered through each gate (node). Note that the tool may not be able to identify $\rho_{max}$ paths through all nodes.
    \item $n_{s}$: The total number of $RVS$ that will be simulated by VADF while attempting to find $\rho_{max}$ longest paths through each node. Increasing $n_{s}$ results in a higher likelihood of the tool being able to find $\rho_{max}$ paths for all instances; however, the run time increases as well.
    \item Process variation specifications: The nominal value $NV_i$, the range of variation $\pm n_i\%$ from $NV_i$, and the standard deviation $\sigma_i$ for each parameter $p_i$. 
\end{itemize}
\begin{figure}[t]
  \centering
  \includegraphics[scale=0.30]{Figures/fin_crop_circuitdiag.pdf}
  
  \caption{Critical paths under different $RVS$'s.}
  \vspace{-2em}
  \label{circuitdiag}
\end{figure}
\begin{figure*}[t]
  \centering
  \includegraphics[scale=1]{Figures/fin_crop_phasewise_flowchart.pdf}
  \caption{Flowchart for longest-path selection using VADF.}
  \vspace{-1.2em}
  \label{vadfflow}
\end{figure*}
Fig. \ref{vadfflow} shows the flowchart of the proposed longest path selection method. The following steps are sequentially performed to obtain the test patterns to detect SDDs in the presence of parameter variations. 



%To calculate the propagation delay of a path under different process variation scenarios, we need the information on how the delay of each gate in the path is affected under those variations. For this, we use HSPICE simulations to create a delay fault library which stores the propagation delay of all standard cells when the different CNFET parameters are independently varied. In the fabrication process, let ${p_1, p_2, ...., p_n}$ be $N$ parameters that are prone to variations, with $p_i$ varying in the range $\pm n_i\%$ from its nominal value. Suppose, for simulation, we consider a granularity $g_i\%$ for each parameter. Thus, for the $k^{}$ means $p_i$ is varied through the following values: $[]$ The total number of simulations is then given by: $\sum\nolimits_{p_i}(2n_i+1)/g_i$. For our simulations, we consider five CNFET parameters -- CNT diameter, CNT spacing, gate length, gate width, and oxide thickness. For each parameter, $n_i=20$ and $g_i=1$; thus we perform 205 HSPICE simulations per gate. In each of these simulations, we perform 1000 Monte Carlo iterations, where the value of the parameter $p_i$ is chosen from a random Gaussian distribution with mean, $\mu_i$ and standard deviation $\sigma_i=0.05*\mu_i$  . The calculated propagation delay for each of these simulations is stored in the corresponding delay-library file of the standard cell, and can be used to estimate the delay of the cell within the predefined variation range. Note that the delay fault library needs to be generated once for every standard cell library, and can be used by all designs synthesized using the same cell library.

To calculate the propagation delay of a path under different process variation scenarios, we need to analyze how the delay of each gate in the path is affected under these variations. For this purpose, we use HSPICE simulations to create a delay fault library that stores the propagation delay of all standard cells when the different CNFET parameters are independently varied. In the fabrication process, let ${p_1, p_2, ...., p_N}$ be $N$ parameters that are prone to variations, with $p_i$ varying in the range $\pm n_i\%$ from its nominal value, $NV_i$. Suppose, for simulation, we consider a step size of $g_i\%$ for each parameter. This means that the value of $p_i$ varies in the following steps: $\{[1-\frac{n_i}{100}]\cdot NV_i, [1-\frac{n_i-g_i}{100}]\cdot NV_i, [1-\frac{n_i-2g_i}{100}]\cdot NV_i, ..., NV_i,$ $...,$ $[1+\frac{n_i-g_i}{100}]\cdot NV_i, [1+\frac{n_i}{100}]\cdot NV_i\}$. For a parameter, $p_i$, the total number of steps is thus given by $\lfloor \frac{2n_i+1}{g_i} \rfloor$. For the $k^{th}$ step, we perform 1000 Monte Carlo iterations where the value of $p_i$ is chosen from a random Gaussian distribution with mean, $\mu_{ik}$, as its value in the $k^{th}$ step. Thus, $\mu_{ik}=[1-\frac{n_i-(k-1)g_i}{100}]\cdot NV_i$. The standard deviation $\sigma_{ik}=0.05\cdot \mu_{ik}$. During the Monte Carlo iterations, all the other parameters, $p_{j,j\neq i}$, are kept at their nominal values. The mean value of the propagation delay, $PD_{ik}$ is calculated using HSPICE simulation. \textcolor{black}{This single-parameter variation is considered only for the CNFET delay-library generation to reduce the number of HSPICE simulations required. This assumption is valid because experimental results (Fig. \ref{gatedelayscatter}) show that the gate delay under multiple simultaneous variations ($RVS$) can be predicted with reasonable accuracy by superposing the impact of each individual parameter variation.}\par 

\subsection{CNFET Delay Fault Library Generation}

The total number of Monte Carlo runs is therefore given by $N_{mc}=\sum\nolimits_{p_i}\lfloor \frac{2n_i+1}{g_i} \rfloor$. For our simulations, we consider five CNFET parameters -- CNT diameter, CNT spacing, gate length, gate width, and oxide thickness. For each parameter, $n_i=20$ and $g_i=1$; thus we perform 205 HSPICE simulations per gate. \textcolor{black}{For each gate $G_k$ and parameter $p_i$, the normalized change in the propagation delay (given by $c_{ik}/d_{0k}$) for a $x_{ik}\%$ variation from the nominal value is stored in the corresponding delay-library file. Simulation results (see Fig. \ref{gatedelayscatter}) show that the $c_{ik}$ values can be used to estimate the delay of the cell within the predefined variation range. The delay fault library needs to be generated once for each standard cell, and can be used by all designs synthesized using the same cell library.}\par

%SammyBammy \textcolor{red}{Add some lines on how this can be used to predict the propagation delay in the presence of multiple variations.}

\subsection{Preprocessing}


The total number of paths in a design scales exponentially with the number of gates \cite{pomeranz2012metric}. Thus, to reduce runtime, we need to create a preliminary shortlist of ``long" testable paths denoted by $L_0$. A path is considered to be ``long" if the timing slack on the path is a small (user-defined) fraction of the clock period. The final set of paths selected for test generation, denoted by $L_1$, is a subset of $L_0$. To create $L_0$, we have used a commercial static timing analysis (STA) tool to obtain an appropriate set of paths in a netlist and shortlisted them based on the following criteria:
\vspace{-0.25em}
\begin{itemize}[leftmargin=*]
    \item \textcolor{black}{\textbf{Criterion 1}: All the paths in $L_0$ have a nominal slack (in absence of process variations) that is less than a threshold that is determined based on the path profile of the design. Paths with high slack margin are not considered because SDDs on those paths are unlikely to affect the circuit functionality. For our simulations, we have considered paths with nominal slack less than 20\% of the clock period.} 
    \item \textbf{Criterion 2}: All the paths in $L_0$ are ATPG-testable. Using $L_0$, VADF selects a subset $L_1$ of paths that must be tested to cover SDDs at all nodes in the netlist. To ensure the coverage of maximum process variation scenarios, we ensure that all paths recommended for each node are testable. \textcolor{black}{Note that here we do not specifically consider robust or non-robust sensitization. While non-robust tests are prone to fault masking, robust tests may fail to detect a delay fault that is detectable by a non-robust test \cite{pierzynska1995non}. Our goal is to consider critical paths under most random variation scenarios; therefore, we do not limit ourselves only to paths that can be robustly sensitized. Additionally, we generate test patterns to sensitize multiple long paths through each fault site. Thus, it is likely that at least one of these long paths will lead to a robust test.}
\end{itemize}
\vspace{-0.25em}
%Thus, it must be ensured that $L_0$ contains sufficient number of paths through each gate. During this step, the user needs to provide the following inputs that are used as exit conditions while selecting $L_0$ and $L_1$:
%\begin{itemize}
%    \item $\rho_{max}$: The maximum number of paths to be generated through each instance in the netlist. Note that the tool may not be able to find $\rho_{max}$ paths through all the instances.
%    \item $num_{scenes}$: The total number of random process variation scenarios that will be simulated by the VADF tool while attempting to find $\rho_{max}$ longest paths through each instance. Increasing $num_{scenes}$ results in a higher likelihood of the tool being able to find $\rho_{max}$ paths for all instances, however the execution time increases as well.
%\end{itemize}
We first use a commercial synthesis tool to insert scan chains in the netlist. Two-step preprocessing is then performed to generate $L_0$ for the scan-inserted netlist. \par
(1) STA Run: In the first step of the preprocessing flow, we obtain the timing characteristics of the design in the absence of any process variation using a commercial STA tool \textcolor{black}{(Synopsys PrimeTime \cite{synopsys})}. To determine the appropriate rated clock period, we first run STA with a 1 ns clock and observe the slack on the longest path. The clock period is subsequently adjusted for the rest of the flow by considering a 1\% positive slack margin for the longest path. For example, suppose the longest path has a slack $sl_{long}$ ns when a 1 ns rated clock is used. For the rest of the analysis, we use a clock period given by $t_{clk}=1.01\cdot (1-sl_{long})$ ns. \par
Next, we rerun the STA tool iteratively using a clock with period \textcolor{black}{$t_{clk}$} and obtain the set of longest paths. In each iteration, the following STA inputs are modified until the number of paths in the list remains constant for consecutive iterations: 
\vspace{-0.25em}
\begin{itemize}[leftmargin=*]
    \item \textit{num\_paths}: The maximum number of long paths generated by the STA tool. In our flow, the starting value of \textit{num\_paths} is equal to the number of instances in the netlist. In each subsequent iteration, we increase the value by 20\%.
    \item \textit{nworst}: The maximum number of paths ending at each scan flop. In our flow, the starting value of \textit{nworst} is equal to (number of instances/50). For each subsequent iteration, we increase \textit{nworst} by 20\%.
    \item \textit{max\_slack}: The maximum slack among all the paths generated. In our flow, we keep it fixed at $0.2\times t_{clk}$. 
\end{itemize}
\vspace{-0.25em}
%Paths generated from the STA tool are written to a report (.rpt) file in increasing order of slack margin. \par
(2) Shortlisting of Testable Long Paths, $L_0$: After the STA run, path delay faults are added to each path and using \textcolor{black}{Synopsys TetraMAX \cite{synopsys}}, the ATPG-Untestable path-delay faults are identified and the corresponding paths are removed from the path list. Therefore, all the paths in the final list satisfy both Criterion 1 and Criterion 2.
\subsection{Selection of Longest Paths for Random Variation Scenarios}
The propagation delay of each \textcolor{black}{path} in $L_0$ is calculated for a total of $n_{s}$ random variation scenarios. In any given variation scenario, for each gate, the CNFET process parameter $p_i$ is randomly chosen from a Gaussian distribution with mean $\mu_i$ as its nominal value and standard deviation $\sigma_i$, and the distribution truncated in the range $[(1-n_i/100)\cdot\mu_i, (1+n_i/100)\cdot\mu_i]$. The process parameters for each gate are chosen randomly independent of the placement of the gate; this ensures that both inter- and intra-die variations are taken into account. As the selection procedure for paths to detect delay faults is independent of the placement, the proposed method needs to be executed only once, even if there are multiple place-and-route iterations. However as mentioned previously, all the transistors in a gate have been assumed to have similar variations in any specific scenario. \par
The CNFET delay fault library is used to calculate the propagation delay of the logic gates under the different variation scenarios. Consider a gate $G_k$ with a nominal delay $d_{0k}$ and process parameters $p_1, p_2, ..., p_n$. The delay contribution of the process parameter $p_i$ is given by $c_{ik}=d_{ik}-d_{0k}$, where $d_{ik}$ is the gate delay in the presence of variation in $p_i$ as obtained from the delay-library. The gate delay in the presence of simultaneous variations in CNFET parameters can be approximated by $D=d_{0k}+\sum\nolimits_{p_i}c_{ik}$. The total delay of a path in a variation scenario is obtained by adding the gate delays of the standard cells in the path. \par
Once the delays of the paths in $L_0$ are calculated for the $n_{s}$ scenarios, a subset of paths, $L_1$, is selected for test generation. For each standard cell, the paths through the cell are sequentially added to $L_1$ and removed from $L_0$ in descending order of propagation delay until one of the following happens: (i) $L_1$ contains $\rho_{max}$ paths through the cell; (ii) there are no paths through the cell remaining in $L_0$. At this point, the path-selection procedure terminates. The number of iterations for long-path selection is $O(n_s\cdot \left|L_0\right|)$. The actual number of iterations required approaches this limit as $\rho_{max}$ increases.
\subsection{Test Generation for Selected Long Paths}
We use a commercial ATPG tool in the Launch-On Shift timing mode to generate test patterns to detect delay faults through the selected paths in $L_1$. \textcolor{black}{Based on the steps for longest path selection, the SDD ATPG flow using VADF can be divided into four phases as shown in Fig. \ref{vadfflow}: P1: Pre-processing step to shortlist long testable paths (see IV.B), P2: Generating $n_s$ $RVS$ (see IV.C), P3: Calculate delay of each shortlisted path in $L_0$ for $n_s$ $RVS$ and select the final list of paths $L_1$ (see IV.C), P4: Test generation for selected long paths (see IV.D). The delay-library generation (Flow A in Fig. \ref{vadfflow}) is not included in these four phases as it needs to be performed only once for each standard cell library.}
